Playing with Repetitions in Data Words Using Energy Games

We introduce two-player games which build words over infinite alphabets, and we study the problem of checking the existence of winning strategies. These games are played by two players, who take turns in choosing valuations for variables ranging over an infinite data domain, thus generating multi-attributed data words. The winner of the game is specified by formulas in the Logic of Repeating Values, which can reason about repetitions of data values in infinite data words. We prove that it is undecidable to check if one of the players has a winning strategy, even in very restrictive settings. However, we prove that if one of the players is restricted to choose valuations ranging over the Boolean domain, the games are effectively equivalent to single-sided games on vector addition systems with states (in which one of the players can change control states but cannot change counter values), known to be decidable and effectively equivalent to energy games. Previous works have shown that the satisfiability problem for various variants of the logic of repeating values is equivalent to the reachability and coverability problems in vector addition systems. Our results raise this connection to the level of games, augmenting further the associations between logics on data words and counter systems.

==> app-dec-singlesided-nestedpast.tex <==
\begin{lem}
    \label{lem:repValuesToVASSNested}
    Let $\phi$ be a \pmainlogic$[\langle \previous, \since\rangle,
    \oblieqlocal, \leftarrow]$ formula with $\dvars^{e} = \bvars^{s} =
    \emptyset$.  If \sys has a winning strategy in the corresponding
    single-sided \pmainlogic$[\langle \previous, \since\rangle,
    \oblieqlocal, \leftarrow]$ game, then she has a winning strategy in
    the single-sided VASS game constructed above.
\end{lem}
\begin{proof}
    Suppose that \sys has a strategy $\ts: \vals^{*}\cdot
    \vals^{e} \to \vals^{s}$ in the single-sided \pmainlogic$[\langle \previous, \since\rangle,
    \oblieqlocal, \leftarrow]$ game. We will show that \sys
    has a strategy $\ssys: (Q \times \Nat^{C})^{*} \cdot (Q^{s}
    \times \Nat^{C}) \to T$ in the single-sided VASS game. It is
routine to construct such a strategy from the mapping $\mu:
(\pwrset(\bvars^{\phi}))^* \to \symbvals \cup \set{\bot}$ that we
define now. For every sequence $\chi \in (\pwrset(\bvars^{\phi}))^*$,
we will define $\mu(\chi)$ and a concrete
model of length $|\chi|$, by induction on $|\chi|$. For the base case
$|\chi|=0$, the concrete model is the empty sequence and
$\mu(\chi)$ is $\bot$.

    For the induction step, suppose $\chi$ is of
    the form $\chi' \cdot V$ and $\sigma$ is the concrete
    model defined for $\chi'$ by induction hypothesis. Let $\upsilon^{e}:\bvars^{e} \to
    \set{\top, \bot}$ be the mapping defined as $\upsilon^{e}(p) =
    \top$ iff $p \in V$. The \sys's strategy $\ts$ in the
    single-sided \pmainlogic$[\top$, $\oblieqlocal$, $\leftarrow]$
    game will give a valuation $\ts(\sigma \cdot \upsilon^{e}) = \upsilon^{s}:
    \dvars^{s} \to \Domain$. We define the finite concrete model
    to be $\sigma \cdot (\upsilon^{e} \oplus \upsilon^{s})$ and
    $\mu(\chi)$ to be the $(\lceil |\sigma| \rceil l, \phi)$-frame $\symbval'$ such that
    $\Omega_{\symbval'} = \set{\phi' \in \Omega^{\phi}_{l} \mid \sigma
    \cdot (\upsilon^{e} \oplus \upsilon^{s}), |\sigma|+1-\lceil
    |\sigma| \rceil l \models \phi'}$. Suppose
    $\mu(\chi')=\symbval$. Then we define
    $H_{\symbval'}(x,e-1)=H_{\symbval}(x,e)$ and
    $\Phi_{\symbval'}(e-1)=\Phi_{\symbval}(e)$ for every $e \in
    [1,\lceil |\sigma| \rceil l]$ and every $x \in \dvars^{\phi}$. We
    define $\Phi_{\symbval'}(\lceil |\sigma| \rceil l)$ to be the set
    $\set{\psi \in \closure(\Phi) \mid \sigma
    \cdot (\upsilon^{e} \oplus \upsilon^{s}), |\sigma|+1 \models
    \psi}$. Let $d \in \Domain$ and $\mathit{pos}(\sigma,d)$ be the set
    $\set{i \in [1,|\sigma|] \mid \sigma(i)(x)=d \text{ for some } x \in
    \dvars^{\phi}}$ of positions of $\sigma$ in which at least one
    variable is assigned to $d$. For every $x \in \dvars^{\phi}$, we
    define $H_{\symbval'}(x,\lceil |\sigma| \rceil l)$ to be the
    repetition history $\cup_{i \in
        \mathit{pos}(\sigma,\upsilon^{s}(x))}\set{(  \set{y \in
            \dvars^{\phi} \mid \sigma(i)(y)=\upsilon^{s}(x)},
            \set{ \psi \in \Phi \mid \sigma,i \models \psi} )}$.

    It is routine to verify that the frame $\symbval'$ defined above
    indeed satisfies all the conditions (F1)--(F10). Intuitively,
    $\Omega_{\symbval'}$ is the set of atomic constraints in
    $\Omega_{l}^{\phi}$ that are satisfied at the position $|\sigma|+1-\lceil
    |\sigma| \rceil l$ of the concrete model $\sigma
    \cdot (\upsilon^{e} \oplus \upsilon^{s})$. The definition of
    $H_{\symbval'}(x,e-1)$ and $\Phi_{\symbval'}(e-1)$ are borrowed
    from the previous frame. We have defined $\Phi_{\symbval'}(\lceil
    |\sigma| \rceil l)$ to be the set of all formulas in
    $\closure(\Phi)$ that are true in the last position of the
    concrete model $\sigma \cdot (\upsilon^{e} \oplus \upsilon^{s})$.
    The repetition history $H_{\symbval'}(x,\lceil |\sigma| \rceil l)$
    is obtained by looking at all the positions in $\sigma$ that
    assigns at least one variable to the data value
    $\upsilon^{s}(x)$, which are all the positions where the data
    value of $x$ at position $|\sigma|+1$ repeats in the past. This
    step crucially uses the fact that nested formulas do not refer to
    future positions --- if they did, we couldn't have constructed the
    frame $\symbval'$ by looking only at the past positions of the
    concrete model.

    Next we will prove that the strategy $\ssys$ defined above is
    winning for \sys. Suppose \sys{} plays
    according to $\ssys$ in the single-sided VASS game, resulting in
    the sequence of states 
    \begin{align*}
        (-1, q^{\phi}_{\init}, \bot) (-1,
        q^{\phi}_{\init}, \bot, V_{1}) (0, q^{\phi}_{\init},
        \symbval_{1}) (0, q^{\phi}_{\init}, \symbval_{1}, V_{2})\\
        (1,q^{\phi}_{\init}, \symbval_{2}) \cdots (l, q, \symbval_{l+1})
        (l,q,\symbval_{l+1}, V_{l+2}) (l,q',\symbval_{l+2}) \cdots
    \end{align*}
    The sequence $\symbval_{l+1} \symbval_{l+2} \cdots$ is an infinite
    $(l,\phi)$-symbolic model; call it $\rho$. It is clear from the construction
    that $\rho$ is realized by a concrete model $\sigma$, which is the
    result of \sys{} playing according to the winning
    strategy $\ts$ in the \pmainlogic$[\langle \previous, \since\rangle,
    \oblieqlocal, \leftarrow]$ game. So $\sigma,1 \models \phi$ and by
    Lemma~\ref{lem:symbolicToConcreteSatNested} (symbolic vs.~concrete
    models), $\rho$ symbolically satisfies $\phi$. By definition of
    $A^{\phi}$, the unique run of $A^{\phi}$ on $\rho$ satisfies the
    parity condition and hence the play satisfies the parity condition in the
    single-sided VASS game. It remains to prove that if a transition
    given by $\ssys$ decrements some counter, that counter will have
    sufficiently high value. Any play starts with all counters
    having zero and a counter is decremented by a transition if the
    frame chosen by that transition has points of decrement for the
    counter. For $e \in \set{1, \ldots, l+1}$ and
    $x \in \dvars^{\phi}$, $[(x,e)]_{\symbval_{e}}$ cannot be a point
    of decrement in $\symbval_{e}$ --- if it were, the data value
    $\sigma(e)(x)$ would have appeared in some position in
    $\set{1, \ldots, e-1}$, creating a backward reference from
    $(x,e)$ in $\symbval_{e}$.

    For $i > l+1$, $x \in \dvars^{\phi}$ and $H \in \RH$, suppose
    $[(x,l)]_{\symbval_{i}}$ is a point of decrement for $H$ in
    $\symbval_{i}$. Before decrementing the counter $H$, it is
    incremented for every point of increment for $H$ in every frame
    $\symbval_{j}$ for all $j < i$. Hence, it suffices to associate with
    this point of decrement a point of
    increment for $H$ in a frame earlier than $\symbval_{i}$ that is
    not associated to any other point of decrement. Since
    $[(x,l)]_{\symbval_{i}}$ is a point of decrement for $H$ in
    $\symbval_{i}$, the data value $\sigma(i)(x)$ appears
    in some of the positions $\set{1, \ldots, i-l-1}$. Let $i' =
    \max\set{j \in \set{1, \ldots, i-l-1} \mid \exists y \in
    \dvars^{\phi}, \sigma(j)(y) = \sigma(i)(x)}$. Let $x' \in
    \dvars^{\phi}$ be such that $\sigma(i')(x') = \sigma(i)(x)$ and associate with
    $[(x,l)]_{\symbval_{i}}$ the class $[(x',0)]_{\symbval_{i'+l}}$,
    which is a point of increment for $H$ in $\symbval_{i'+l}$. The
    class $[(x',0)]_{\symbval_{i'+l}}$ cannot be associated with any
    other point of decrement for $H$ --- suppose it were associated with
    $[(y,l)]_{\symbval_{j}}$, which is a point of decrement for
    $H$ in $\symbval_{j}$. Then $\sigma(j)(y) = \sigma(i)(x)$. If
    $j = i$, then $[(x,l)]_{\symbval_{i}} = [(y,l)]_{\symbval_{j}}$
    and the two points of decrement are the same. So $j < i$ or
    $j>i$. We compute $j'$ for $[(y,l)]_{\symbval_{j}}$ with
    $j' < j$ just like we computed $i'$ for $[(x,l)]_{\symbval_{i}}$.
    If $j < i$, then $j$ would be one of the positions in $\set{1,
    \ldots, i-l-1}$
    where the data value
    $\sigma(i)(x)$ appears ($j$ cannot be in the interval $[i-l, i-1]$
    since those positions do not contain the data value
    $\sigma(i)(x)$; if they did, there would have been a backward
    reference from $(x,l)$ in $\symbval_{i}$ and
    $[(x,l)]_{\symbval_{i}}$ would not have been a point of decrement), so
    $j \le i'$ (and hence $j' < i'$). If $j > i$, then $i$ is one of
    the positions in $\set{1, \ldots, j-l-1}$ where the data value
    $\sigma(j)(y)$ appears ($i$ cannot be in the interval $[j-l, j-1]$
    since those positions do not contain the data value
    $\sigma(j)(y)$; if they did, there would have been a backward
    reference from $(y,l)$ in $\symbval_{j}$ and
    $[(y,l)]_{\symbval_{j}}$ would not have been a point of decrement), so $i \le j'$ (and hence $i' < j'$). In
    both cases, $j' \ne i'$ and hence, the class
    $[y',0]_{\symbval_{j'+l}}$ we associate with
    $[(y,l)]_{\symbval_{j}}$ would be different from
    $[(x',0)]_{\symbval_{i'+l}}$.
\end{proof}

\begin{lem}
    \label{lem:VASSTorepValuesNested} Let $\phi$ be a
    \pmainlogic$[\langle \previous, \since\rangle, \oblieqlocal,
    \leftarrow]$ formula with $\dvars^{e} = \bvars^{s} = \emptyset$.
    If \sys has a winning strategy in the single-sided VASS game
    constructed above, then she has a winning strategy in the
    corresponding single-sided \pmainlogic$[\langle \previous,
    \since\rangle, \oblieqlocal, \leftarrow]$ game.
\end{lem}
\begin{proof}
    Suppose \sys{} has a strategy $\ssys: (Q \times
    \Nat^{C})^{*} \cdot (Q^{s} \times \Nat^{C}) \to T$ in the
    single-sided VASS game. We will show that \sys{} has a
    strategy $\ts: \vals^{*}\cdot \vals^{e} \to \vals^{s}$ in the
    single-sided \pmainlogic$[\langle \previous, \since\rangle, \oblieqlocal,
    \leftarrow]$
    game. For every $\sigma \in \vals^{*}$ and every $\val^{e} \in
    \vals^{e}$, we will define $\ts(\sigma \cdot \val^{e}):
    \dvars^{\phi} \to \Domain$ and a sequence of configurations
    $\chi \cdot ((e,q,\symbval),\vec{n}_{\inc} - \vec{n}_{\dec})$ in
    $(Q \times \Nat^{C})^{*}\cdot (Q^{e}\times\Nat^{C})$ of length
    $2|\sigma|+3$ such that for every repetition history $H \in
    \RH$, $\vec{n}_{\inc}(H)$ is the sum of the
    number of points of increment for $H$ in all the frames occurring
    in $\chi$ and $\vec{n}_{\dec}(H)$ is the sum of the number of points
    of decrement for $H$ in all the frames occurring in $\chi$ and in
    $\symbval$. We will do this by induction on
    $|\sigma|$ and prove that the resulting strategy is winning for the
    system player. By \emph{frames occurring in $\chi$}, we refer to
    frames $\symbval$ such that there are consecutive configurations
    $( (e, q, \symbval), \vec{n}) ( (e,q,\symbval,V), \vec{n})$ in
    $\chi$. By $\Pi_{\symbvals}(\chi)(i)$, we refer to
    $i$\textsuperscript{th} such occurrence of a frame in $\chi$. Let
    $\set{d_{0}, d_{1}, \ldots} \subseteq \Domain$ be a countably
    infinite set of data values.

    For the base case $|\sigma|=0$, let $V \subseteq \bvars^{e}$ be
    defined as $p \in V$ iff $\val^{e}(p)=\top$. Let $\ssys((
    (-1, q^{\phi}_{\init},\bot),\vec{0})\cdot((-1,
    q^{\phi}_{\init},\bot,V),\vec{0}))$ be the transition $(-1,
    q^{\phi}_{\init},\bot,V) \act{\vec{0}-\dec(\symbval_{1})} (0, q,
    \symbval_{1})$. Since $\ssys$ is a winning strategy for \sys in
    the single-sided VASS game, $\dec(\symbval_{1})$ is necessarily
    equal to $\vec{0}$. The
    set of variables $\dvars^{\phi}$ is partitioned into equivalence
    classes by the $(0,\phi)$-frame $\symbval_{1}$. We define
    $\ts(\val^{e})$ to be the valuation that assigns to each such
    equivalence class a data value $d_{j}$, where $j$ is the
    smallest number such that $d_{j}$ is not assigned to any variable
    yet. We let the sequence of configurations be $(
    (-1,q^{\phi}_{\init}, \bot),\vec{0}) \cdot
    ( (-1,q^{\phi}_{\init}, \bot, V), \vec{0}) \cdot (
    (0,q,\symbval_{1}), -\dec(\symbval_{1}))$.
    %\sidediego{Do we need to say that $\dec(\symbval_{1}) = 0$ necessarily?}

    For the induction step, suppose $\sigma\cdot \val^{e} = \sigma'
    \cdot (\val^{e}_{1}\oplus \val^{s}_{1} ) \cdot \val^{e}$ and
    $\chi' \cdot ((e,q,\symbval), \vec{n})$ is the sequence of
    configurations given by the induction hypothesis for $\sigma'
    \cdot \val^{e}_{1}$. If $\set{\phi' \in \Omega^{\phi}_{l} \mid
    \sigma' \cdot (\val^{e}_{1} \oplus \val^{s}_{1}),|\sigma'|+1-e
    \models \phi'} \ne \Omega_{\symbval}$, it corresponds to the case where the
    system player in the \pmainlogic$[\langle \previous, \since\rangle, \oblieqlocal,
    \leftarrow]$ game has already deviated from the strategy we have
    defined so far. So in this case, we define $\ts(\sigma\cdot
    \val^{e})$ and the sequence of configurations to be arbitrary.
    Otherwise, we have $\set{\phi' \in \Omega^{\phi}_{l} \mid
    \sigma' \cdot (\val^{e}_{1} \oplus \val^{s}_{1}),|\sigma'|+1-e
    \models \phi'} = \Omega_{\symbval}$. Let $V \subseteq \bvars^{e}$ be
    defined as $p \in V$ iff $\val^{e}(p)=\top$ and let $\ssys( \chi' \cdot (
    (e,q,\symbval),\vec{n}) \cdot  ((e,q,\symbval,V),\vec{n}))$ be the
    transition $(e,q,\symbval,V) \act{\inc(\symbval) - \dec(\symbval')} (\lceil e+1 \rceil l, q',
    \symbval')$. We define the sequence of configurations as
    $\chi'\cdot ((e,q,\symbval), \vec{n}) \cdot ( (e,q,\symbval,V)
    \vec{n}) \cdot ((\lceil e+1 \rceil l, q',\symbval'),
    \vec{n} + \inc(\symbval) - \dec(\symbval'))$. Since $\ssys$ is a
    winning strategy for the system player in the single-sided VASS
    game, $ \vec{n} + \inc(\symbval) - \dec(\symbval') \ge
    \vec{0}$. The valuation $\ts(\sigma \cdot
    \val^{e}): \dvars^{\phi} \to \Domain$ is defined as follows. The
    set $\dvars^{\phi}$ is partitioned into
    equivalence classes at level $\lceil e+1 \rceil l$ in
    $\symbval'$. For every such equivalence class $[(x,\lceil e+1
    \rceil l)]_{\symbval'}$, assign the data value $d'$ as defined
    below.
    \begin{enumerate}
        \item If there is a backward reference $\mynext^{\lceil e+1
            \rceil l}x \oblieqlocal \mynext^{\lceil e+1 \rceil l -j}y$ in
            $\symbval'$, let $d' = \sigma'\cdot (\val^{e}_{1} \oplus
            \val^{s}_{1})(|\sigma'|+2-j)(y)$.
        \item If there are no backward references from $(x,\lceil e+1
            \rceil l)$ in $\symbval'$ and the set
            $\pobli_{\symbval}(x,\lceil e+1 \rceil l)$ of past
            obligations of $x$ at level $\lceil e+1 \rceil l$ in
            $\symbval'$ is empty, let $d'$ be $d_{j}$, where $j$ is
            the smallest number such that $d_{j}$ is not assigned to
            any variable yet.
        \item If there are no backward references from $(x,\lceil e+1
            \rceil l)$ in $\symbval'$ and the set
            $O=\pobli_{\symbval}(x,\lceil e+1 \rceil l)$ of past
            obligations of $x$ at level $\lceil e+1 \rceil l$ in
            $\symbval'$ is non-empty, then $[(x,\lceil e+1
            \rceil l)]_{\symbval'}$ is a point of decrement for the
            repetition history
            $H=H_{\symbval'}(x,\lceil e+1 \rceil l)$ in
            $\symbval'$. Pair off this with a point of increment for
            $H_{\symbval'}(x,\lceil e+1 \rceil l)$ in a frame that occurs in $\chi' \cdot (
            (e,q,\symbval),\vec{n}) \cdot  ((e,q,\symbval,V),\vec{n})$
            that has not been paired off before. It is possible to do
            this for every point of decrement for $H$ in $\symbval'$,
            since $(\vec{n} + \inc(\symbval))(H)$ is the number of
            points of increment for $H$  occurring in $\chi' \cdot (
            (e,q,\symbval),\vec{n}) \cdot  ((e,q,\symbval,V),\vec{n})$
            that have not yet been paired off and $(\vec{n} +
            \inc(\symbval))(H) \ge \dec(\symbval')(H)$ for every
            repetition history $H$. Suppose we
            pair off $[(x,\lceil e+1 \rceil l)]_{\symbval'}$ with a
            point of increment $[(y,0)]_{\symbval_{i}}$ in the frame
            $\symbval_{i} = \Pi_{\symbvals}(\chi' \cdot (
            (e,q,\symbval),\vec{n}) \cdot
            ((e,q,\symbval,V),\vec{n}))(i)$, then let $d'$ be
            $\sigma'\cdot (\val^{e}_{1} \oplus \val^{s}_{1})(i)(y)$.
            From the definition of the repetition history $\rh$ matching
            the set $\po$ of past obligations
            (page \pageref{matching-second-condition}), we infer that for every
            variable $z$ such that the data value $d'$ is assigned to
            $z$ at some past position that satisfies some nested
            formula $\psi \in \Phi$, $\Omega_{\symbval'}$ contains the
            formula $\mynext^{\lceil e+1 \rceil
            l}(\oblieqp{x}{z}{\psi})$. This ensures that
            $\Omega_{\symbval'}$ contains \emph{all} the past
            repetitions of $d'$, which is required to ensure that the
            concrete model we build realizes the sequence of frames
            that we identify next.
    \end{enumerate}
    Suppose the system player plays according to the strategy
    $\ts$ defined above, resulting in the model
    $\sigma = (\val^{e}_{1} \oplus \val^{s}_{1}) \cdot (\val^{e}_{2} \oplus
    \val^{s}_{2}) \cdots$. It is clear from the construction that
    there is a sequence of configurations 
    \begin{align*}
        ((-1, q^{\phi}_{\init}, \bot), \vec{0}) ((-1,
        q^{\phi}_{\init}, \bot, V_{1}), \vec{0})\\ ((0, q^{\phi}_{\init},
        \symbval_{1}), \vec{n}_{1}) ((0, q^{\phi}_{\init},
        \symbval_{1}, V_{2}), \vec{n}_{1})\\
        ((1,q^{\phi}_{\init}, \symbval_{2}), \vec{n}_{2}) \cdots ((l,
        q, \symbval_{l+1}), \vec{n}_{l+1})\\
        ((l,q,\symbval_{l+1}, V_{l+2}), \vec{n}_{l+1})
        ((l,q',\symbval_{l+2}), \vec{n}_{l+2}) \cdots
    \end{align*}
    that is the result of the system player playing according to the
    strategy $\ssys$ in the single-sided VASS game such that the
    concrete model $\sigma$ realizes the symbolic model
    $\symbval_{l+1} \symbval_{l+2} \cdots$. Since $\ssys$ is a winning
    strategy for the system player, the sequence of configurations
    above satisfy the parity condition of the single-sided VASS game,
    so $\symbval_{l+1} \symbval_{l+2} \cdots$ symbolically satisfies
    $\phi$. From Lemma~\ref{lem:symbolicToConcreteSatNested} (symbolic
    vs.~concrete models), we conclude that $\sigma$ satisfies
    $\phi$.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> app-single-past-decidable.tex <==
\subsection{Proof details for the forward direction of Lemma~\ref{lem:repValuesToVASS}}
    Suppose the system player has a strategy $\ts: \vals^{*}\cdot
    \vals^{e} \to \vals^{s}$ in the single-sided \pmainlogic$[\top$,
    $\oblieqlocal$, $\leftarrow]$ game. We will show that the system
    player has a strategy $\ssys: (Q \times \Nat^{C})^{*} \cdot (Q^{s}
    \times \Nat^{C}) \to T$ in the single-sided VASS game. It is
routine to construct such a strategy from the mapping $\mu:
(\pwrset(\bvars^{\phi}))^* \to \symbvals \cup \set{\bot}$ that we
define now. For every sequence $\chi \in (\pwrset(\bvars^{\phi}))^*$,
we will define $\mu(\chi)$ and a concrete
model of length $|\chi|$, by induction on $|\chi|$. For the base case
$|\chi|=0$, the concrete model is the empty sequence and the frame is
$\bot$.
    %For every
    %$\chi \in (Q \times \Nat^{C})^{*}$ and every $(q^s,\vec{n}) \in
    %Q^{s} \times \Nat^{C}$, we will define $\ssys(\chi \cdot
    %(q^s,\vec{n}))$ and a finite concrete model whose length is equal to the
    %number of system states in $\chi\cdot (q^s, \vec{n})$. We
    %will do this by induction on $|\chi|$ and prove that the resulting
    %strategy is winning for the system player.

    %For defining the strategy $\ssys$, some cases are not important
    %since they will not arise when the system player plays according
    %to $\ssys$. Hence for these cases, we leave the strategy
    %definition to be arbitrary. The first such case is when the
    %initial configuration in $\chi$ does not have all the counters initialized
    %to zero. The case where there are two consecutive configurations
    %$( (e,q,\symbval, V), \vec{n}) ( (\lceil e+1 \rceil l , q',
    %\symbval'), \vec{n'})$ in $\chi$ can be similarly
    %ignored if there is no transition $(e,q,\symbval, V)
    %\act{\vec{n'} - \vec{n}} (\lceil e+1 \rceil l , q',
    %\symbval')$. The next case is the base case
    %$|\chi|=0$ (here the play starts at the system state
    %$q$, but we have defined the initial state to be the environment
    %state $(-1, q^{\phi}_{\init}, \bot)$), where we define the concrete model to be the empty
    %sequence $\epsilon$. Another unimportant case is when $(\chi \cdot
    %(q, \vec{n}))$ is not of the form $\chi' \cdot (
    %(e,q,\symbval),\vec{n}) \cdot ( (e,q,\symbval, V),\vec{n})$.
    %Another case is when $(\chi \cdot
    %(q, \vec{n}))$ is of the form $\chi' \cdot (
    %(e,q,\symbval),\vec{n}) \cdot ( (e,q,\symbval, V),\vec{n})$,
    %$e=-1$ but $\symbval \ne \bot$ or $q \ne q^{\phi}_{\init}$.
    %Another case is when $(\chi \cdot
    %(q, \vec{n}))$ is of the form $\chi' \cdot (
    %(e,q,\symbval),\vec{n}) \cdot ( (e,q,\symbval, V),\vec{n})$,
    %$e \ge 0$ but $\symbval
    %\ne \set{\phi' \in \Omega^{\phi}_{l} \mid \sigma, |\sigma|-e
    %\models \phi'}$, where $\sigma$ is the concrete model given by the
    %induction hypothesis for $\chi'$.
    %Suppose $q$ is of the form $(-1, q^{\phi}_{\init}, \bot,
    %V)$ (all possible successors are of this form). Let
    %$\upsilon^{e}:\bvars^{e} \to \set{\top, \bot}$ be the mapping
    %defined as $\upsilon^{e}(p) = \top$ iff $p \in V$. The system
    %player's strategy $\ts$ in the single-sided \pmainlogic$[\top$,
    %$\oblieqlocal$, $\leftarrow]$ game will give a valuation
    %$\ts(\upsilon^{e}) = \upsilon^{s}: \dvars^{s} \to \Domain$. We define the finite
    %concrete model $\sigma$ to be the model $(\upsilon^{e} \oplus
    %\upsilon^{s})$ of length one. Let $\symbval'$ be the
    %$(0,\phi)$-frame $\set{\phi' \in \Omega^{\phi}_{l} \mid \sigma,1
    %\models \phi'}$. We define $\ssys( (q,\vec{n}))$ to be the transition
    %$(-1,q^{\phi}_{\init},\bot,V) \act{-\dec(\symbval')} (0,
    %q^{\phi}_{\init},\symbval')$. If $q$ is not of the form $(-1, q^{\phi}_{\init}, \bot,
    %V)$, we define the concrete model and $\ssys( (q,\vec{n}))$
    %arbitrarily.

    For the induction step, suppose $\chi$ is of
    the form $\chi' \cdot V$ and $\sigma$ is the concrete
    model defined for $\chi'$ by induction hypothesis. Let $\upsilon^{e}:\bvars^{e} \to
    \set{\top, \bot}$ be the mapping defined as $\upsilon^{e}(p) =
    \top$ iff $p \in V$. The system player's strategy $\ts$ in the
    single-sided \pmainlogic$[\top$, $\oblieqlocal$, $\leftarrow]$
    game will give a valuation $\ts(\sigma \cdot \upsilon^{e}) = \upsilon^{s}:
    \dvars^{s} \to \Domain$. We define the finite concrete model
    to be $\sigma \cdot (\upsilon^{e} \oplus \upsilon^{s})$ and
$\mu(\chi)$ to be the
    frame
    $\symbval' = \set{\phi' \in \Omega^{\phi}_{l} \mid \sigma \cdot
    (\upsilon^{e} \oplus \upsilon^{s}), |\sigma|+1-\lceil |\sigma| \rceil l
    \models \phi'}$.

    Next we will prove that the strategy $\ssys$ defined above is
    winning for the system player. Suppose the system player plays
    according to $\ssys$ in the single-sided VASS game, resulting in
    the sequence of states 
    \begin{align*}
        (-1, q^{\phi}_{\init}, \bot) (-1,
        q^{\phi}_{\init}, \bot, V_{1}) (0, q^{\phi}_{\init},
        \symbval_{1}) (0, q^{\phi}_{\init}, \symbval_{1}, V_{2})\\
        (1,q^{\phi}_{\init}, \symbval_{2}) \cdots (l, q, \symbval_{l+1})
        (l,q,\symbval_{l+1}, V_{l+2}) (l,q',\symbval_{l+2}) \cdots
    \end{align*}
    The sequence $\symbval_{l+1} \symbval_{l+2} \cdots$ is an infinite
    $(l,\phi)$-symbolic model; call it $\rho$. It is clear from the construction
    that $\rho$ is realized by a concrete model $\sigma$, which is the
    result of the system player playing according to the winning
    strategy $\ts$ in the \pmainlogic[$\top$, $\oblieqlocal$,
    $\leftarrow$] game. So $\sigma,1 \models \phi$ and by
    Lemma~\ref{lem:symbolicToConcreteSat} (symbolic vs.~concrete
    models), $\rho$ symbolically satisfies $\phi$. By definition of
    $A^{\phi}$, the unique run of $A^{\phi}$ on $\rho$ satisfies the
    parity condition and hence the play satisfies the parity condition in the
    single-sided VASS game. It remains to prove that if a transition
    given by $\ssys$ decrements some counter, that counter will have
    sufficiently high value. Any play starts with all counters
    having zero and a counter is decremented by a transition if the
    frame chosen by that transition has points of decrement for the
    counter. For $e \in \set{1, \ldots, l+1}$ and
    $x \in \dvars^{\phi}$, $[(x,e)]_{\symbval_{e}}$ cannot be a point
    of decrement in $\symbval_{e}$ --- if it were, the data value
    $\sigma(e)(x)$ would have appeared in some position in
    $\set{1, \ldots, e-1}$, creating a backward reference from
    $(x,e)$ in $\symbval_{e}$.

    For $i > l+1$, $x \in \dvars^{\phi}$ and $X \in
    \nepwrset(\dvars^{\phi})$, suppose
    $[(x,l)]_{\symbval_{i}}$ is a point of decrement for $X$ in
    $\symbval_{i}$. Before decrementing the counter $X$, it is
    incremented for every point of increment for $X$ in every frame
    $\symbval_{j}$ for all $j < i$. Hence, it suffices to associate with
    this point of decrement a point of
    increment for $X$ in a frame earlier than $\symbval_{i}$ that is
    not associated to any other point of decrement. Since
    $[(x,l)]_{\symbval_{i}}$ is a point of decrement for $X$ in
    $\symbval_{i}$, the data value $\sigma(i)(x)$ appears
    in some of the positions $\set{1, \ldots, i-l-1}$. Let $i' =
    \max\set{j \in \set{1, \ldots, i-l-1} \mid \exists y \in
    \dvars^{\phi}, \sigma(j)(y) = \sigma(i)(x)}$. Let $x' \in
    X$ be such that $\sigma(i')(x') = \sigma(i)(x)$ and associate with
    $[(x,l)]_{\symbval_{i}}$ the class $[(x',0)]_{\symbval_{i'+l}}$,
    which is a point of increment for $X$ in $\symbval_{i'+l}$. The
    class $[(x',0)]_{\symbval_{i'+l}}$ cannot be associated with any
    other point of decrement for $X$ --- suppose it were associated with
    $[(y,l)]_{\symbval_{j}}$, which is a point of decrement for
    $X$ in $\symbval_{j}$. Then $\sigma(j)(y) = \sigma(i)(x)$. If
    $j = i$, then $[(x,l)]_{\symbval_{i}} = [(y,l)]_{\symbval_{j}}$
    and the two points of decrement are the same. So $j < i$ or
    $j>i$. We compute $j'$ for $[(y,l)]_{\symbval_{j}}$ with
    $j' < j$ just like we computed $i'$ for $[(x,l)]_{\symbval_{i}}$.
    If $j < i$, then $j$ would be one of the positions in $\set{1,
    \ldots, i-l-1}$
    %\sidediego{One should also argue that it is not
    %the case that  $j-l-1 < i < j$.}
    where the data value
    $\sigma(i)(x)$ appears ($j$ cannot be in the interval $[i-l, i-1]$
    since those positions do not contain the data value
    $\sigma(i)(x)$; if they did, there would have been a backward
    reference from $(x,l)$ in $\symbval_{i}$ and
    $[(x,l)]_{\symbval_{i}}$ would not have been a point of decrement), so
    $j \le i'$ (and hence $j' < i'$). If $j > i$, then $i$ is one of
    the positions in $\set{1, \ldots, j-l-1}$ where the data value
    $\sigma(j)(y)$ appears ($i$ cannot be in the interval $[j-l, j-1]$
    since those positions do not contain the data value
    $\sigma(j)(y)$; if they did, there would have been a backward
    reference from $(y,l)$ in $\symbval_{j}$ and
    $[(y,l)]_{\symbval_{j}}$ would not have been a point of decrement), so $i \le j'$ (and hence $i' < j'$). In
    both cases, $j' \ne i'$ and hence, the class
    $[y',0]_{\symbval_{j'+l}}$ we associate with
    $[(y,l)]_{\symbval_{j}}$ would be different from
    $[(x',0)]_{\symbval_{i'+l}}$.
    %Suppose $X \in \nepwrset(\dvars^{\phi})$
    %is a counter. There is a possibility that the counter goes below
    %zero during some transition if there is a point of decrement in
    %the frame chosen by that
    %transition. For frames $\symbval_{l+1}$ or before, this can not
    %happen since any
    %repetition of a data value in the past will result in a backward
    %edge and hence there can not be points of decrement. Suppose $i >
    %l + 1$ and there is a point of decrement for $X$ in the frame
    %$\symbval_i$. We will assign to this point of decrement a point of
    %increment, which is not assigned to any other point of decrement.
    %Suppose the point of decrement in $\symbval_i$ is due to a
    %variable $x$, which is assigned a data value $d$ in the concrete
    %model $\sigma$ at position $i$. At the position $\max\set{j \in \set{0, \ldots ,
    %i-l-1} \mid \sigma(j)(y) = d \text{ for some } y \in V}$, there is
    %a point of increment for $X$. This occurs at least $(l + 1)$
    %positions before $i$ (otherwise, there would have been a backward
    %edge from $(x,l)$ in $\symbval_i$ and it would not have been a point
    %of decrement) and hence would result in an increment of the
    %counter $X$ before the point of decrement in $\symbval_i$
    %decrements the counter. In addition, this point of increment is
    %not assigned to any other points of decrement.  If that were to
    %happen, that other point of decrement would also have the data
    %value $d$. That other point of decrement can not be in positions
    %$\set{0, \ldots , i-l-1}$ (such points of decrement would be
    %assigned points of increments at positions earlier than $\max\set{j
    %\in {0, . . . , i - l - 1} \mid \sigma(j)(y) = d \text{ for
    %some } y \in V }$), nor in positions $\set{i-l,...,i-1}$
    %(those positions do not have the data value $d$) and it can
    %not be in positions greater than $i$ (such points of decrement
    %would be assigned points of increments at positions $i$ or
    %later).
\subsection{Proof details for the reverse direction of Lemma~\ref{lem:repValuesToVASS}}
    Suppose the system player has a strategy $\ssys: (Q \times
    \Nat^{C})^{*} \cdot (Q^{s} \times \Nat^{C}) \to T$ in the
    single-sided VASS game. We will show that the system player has a
    strategy $\ts: \vals^{*}\cdot \vals^{e} \to \vals^{s}$ in the
    single-sided \pmainlogic$[\top$, $\oblieqlocal$, $\leftarrow]$
    game. For every $\sigma \in \vals^{*}$ and every $\val^{e} \in
    \vals^{e}$, we will define $\ts(\sigma \cdot \val^{e}):
    \dvars^{\phi} \to \Domain$ and a sequence of configurations
    $\chi \cdot ((e,q,\symbval),\vec{n}_{\inc} - \vec{n}_{\dec})$ in
    $(Q \times \Nat^{C})^{*}\cdot (Q^{e}\times\Nat^{C})$ of length
    $2|\sigma|+3$ such that for every counter $X \in
    \nepwrset(\dvars^{\phi})$, $\vec{n}_{\inc}(X)$ is the sum of the
    number of points of increment for $X$ in all the frames occurring
    in $\chi$ and $\vec{n}_{\dec}(X)$ is the sum of the number of points
    of decrement for $X$ in all the frames occurring in $\chi$ and in
    $\symbval$. We will do this by induction on
    $|\sigma|$ and prove that the resulting strategy is winning for the
    system player. By \emph{frames occurring in $\chi$}, we refer to
    frames $\symbval$ such that there are consecutive configurations
    $( (e, q, \symbval), \vec{n}) ( (e,q,\symbval,V), \vec{n})$ in
    $\chi$. By $\Pi_{\symbvals}(\chi)(i)$, we refer to
    $i$\textsuperscript{th} such occurrence of a frame in $\chi$. Let
    $\set{d_{0}, d_{1}, \ldots} \subseteq \Domain$ be a countably
    infinite set of data values.

    For the base case $|\sigma|=0$, let $V \subseteq \bvars^{e}$ be
    defined as $p \in V$ iff $\val^{e}(p)=\top$. Let $\ssys((
    (-1, q^{\phi}_{\init},\bot),\vec{0})\cdot((-1,
    q^{\phi}_{\init},\bot,V),\vec{0}))$ be the transition $(-1,
    q^{\phi}_{\init},\bot,V) \act{\vec{0}-\dec(\symbval_{1})} (0, q,
    \symbval_{1})$. Since $\ssys$ is a winning strategy for \sys in
    the single-sided VASS game, $\dec(\symbval_{1})$ is necessarily
    equal to $\vec{0}$. The
    set of variables $\dvars^{\phi}$ is partitioned into equivalence
    classes by the $(0,\phi)$-frame $\symbval_{1}$. We define
    $\ts(\val^{e})$ to be the valuation that assigns to each such
    equivalence class a data value $d_{j}$, where $j$ is the
    smallest number such that $d_{j}$ is not assigned to any variable
    yet. We let the sequence of configurations be $(
    (-1,q^{\phi}_{\init}, \bot),\vec{0}) \cdot
    ( (-1,q^{\phi}_{\init}, \bot, V), \vec{0}) \cdot (
    (0,q,\symbval_{1}), -\dec(\symbval_{1}))$.
    %\sidediego{Do we need to say that $\dec(\symbval_{1}) = 0$ necessarily?}

    For the induction step, suppose $\sigma\cdot \val^{e} = \sigma'
    \cdot (\val^{e}_{1}\oplus \val^{s}_{1} ) \cdot \val^{e}$ and
    $\chi' \cdot ((e,q,\symbval), \vec{n})$ is the sequence of
    configurations given by the induction hypothesis for $\sigma'
    \cdot \val^{e}_{1}$. If $\set{\phi' \in \Omega^{\phi}_{l} \mid
    \sigma' \cdot (\val^{e}_{1} \oplus \val^{s}_{1}),|\sigma'|+1-e
    \models \phi'} \ne \symbval$, it corresponds to the case where the
    system player in the \pmainlogic$[\top$, $\oblieqlocal$,
    $\leftarrow]$ game has already deviated from the strategy we have
    defined so far. So in this case, we define $\ts(\sigma\cdot
    \val^{e})$ and the sequence of configurations to be arbitrary.
    Otherwise, we have $\set{\phi' \in \Omega^{\phi}_{l} \mid
    \sigma' \cdot (\val^{e}_{1} \oplus \val^{s}_{1}),|\sigma'|+1-e
    \models \phi'} = \symbval$. Let $V \subseteq \bvars^{e}$ be
    defined as $p \in V$ iff $\val^{e}(p)=\top$ and let $\ssys( \chi' \cdot (
    (e,q,\symbval),\vec{n}) \cdot  ((e,q,\symbval,V),\vec{n}))$ be the
    transition $(e,q,\symbval,V) \act{\inc(\symbval) - \dec(\symbval')} (\lceil e+1 \rceil l, q',
    \symbval')$. We define the sequence of configurations as
    $\chi'\cdot ((e,q,\symbval), \vec{n}) \cdot ( (e,q,\symbval,V)
    \vec{n}) \cdot ((\lceil e+1 \rceil l, q',\symbval'),
    \vec{n} + \inc(\symbval) - \dec(\symbval'))$. Since $\ssys$ is a
    winning strategy for the system player in the single-sided VASS
    game, $ \vec{n} + \inc(\symbval) - \dec(\symbval') \ge
    \vec{0}$. The valuation $\ts(\sigma \cdot
    \val^{e}): \dvars^{\phi} \to \Domain$ is defined as follows. The
    set $\dvars^{\phi}$ is partitioned by the
    equivalences classes at level $\lceil e+1 \rceil l$ in
    $\symbval'$. For every such equivalence class $[(x,\lceil e+1
    \rceil l)]_{\symbval'}$, assign the data value $d'$ as defined
    below.
    \begin{enumerate}
        \item If there is a backward reference $\mynext^{\lceil e+1
            \rceil l}x \oblieqlocal \mynext^{\lceil e+1 \rceil l -j}y$ in
            $\symbval'$, let $d' = \sigma'\cdot (\val^{e}_{1} \oplus
            \val^{s}_{1})(|\sigma'|+2-j)(y)$.
        \item If there are no backward references from $(x,\lceil e+1
            \rceil l)$ in $\symbval'$ and the set
            $\pobli_{\symbval}(x,\lceil e+1 \rceil l)$ of past
            obligations of $x$ at level $\lceil e+1 \rceil l$ in
            $\symbval'$ is empty, let $d'$ be $d_{j}$, where $j$ is
            the smallest number such that $d_{j}$ is not assigned to
            any variable yet.
        \item If there are no backward references from $(x,\lceil e+1
            \rceil l)$ in $\symbval'$ and the set
            $\pobli_{\symbval}(x,\lceil e+1 \rceil l)$ of past
            obligations of $x$ at level $\lceil e+1 \rceil l$ in
            $\symbval'$ is the non-empty set $X$, then $[(x,\lceil e+1
            \rceil l)]_{\symbval'}$ is a point of decrement for $X$ in
            $\symbval'$. Pair off this with a point of increment for
            $X$ in a frame that occurs in $\chi' \cdot (
            (e,q,\symbval),\vec{n}) \cdot  ((e,q,\symbval,V),\vec{n})$
            that has not been paired off before. It is possible to do
            this for every point of decrement for $X$ in $\symbval'$,
            since $(\vec{n} + \inc(\symbval))(X)$ is the number of
            points of increment for $X$  occurring in $\chi' \cdot (
            (e,q,\symbval),\vec{n}) \cdot  ((e,q,\symbval,V),\vec{n})$
            that have not yet been paired off and $(\vec{n} +
            \inc(\symbval))(X) \ge \dec(\symbval')(X)$. Suppose we
            pair off $[(x,\lceil e+1 \rceil l)]_{\symbval'}$ with a
            point of increment $[(y,0)]_{\symbval_{i}}$ in the frame
            $\symbval_{i} = \Pi_{\symbvals}(\chi' \cdot (
            (e,q,\symbval),\vec{n}) \cdot
            ((e,q,\symbval,V),\vec{n}))(i)$, then let $d'$ be
            $\sigma'\cdot (\val^{e}_{1} \oplus \val^{s}_{1})(i)(y)$.
    \end{enumerate}
    Suppose the system player plays according to the strategy
    $\ts$ defined above, resulting in the model
    $\sigma = (\val^{e}_{1} \oplus \val^{s}_{1}) \cdot (\val^{e}_{2} \oplus
    \val^{s}_{2}) \cdots$. It is clear from the construction that
    there is a sequence of configurations 
    \begin{align*}
        ((-1, q^{\phi}_{\init}, \bot), \vec{0}) ((-1,
        q^{\phi}_{\init}, \bot, V_{1}), \vec{0})\\ ((0, q^{\phi}_{\init},
        \symbval_{1}), \vec{n}_{1}) ((0, q^{\phi}_{\init},
        \symbval_{1}, V_{2}), \vec{n}_{1})\\
        ((1,q^{\phi}_{\init}, \symbval_{2}), \vec{n}_{2}) \cdots ((l,
        q, \symbval_{l+1}), \vec{n}_{l+1})\\
        ((l,q,\symbval_{l+1}, V_{l+2}), \vec{n}_{l+1})
        ((l,q',\symbval_{l+2}), \vec{n}_{l+2}) \cdots
    \end{align*}
    that is the result of the system player playing according to the
    strategy $\ssys$ in the single-sided VASS game such that the
    concrete model $\sigma$ realizes the symbolic model
    $\symbval_{l+1} \symbval_{l+2} \cdots$. Since $\ssys$ is a winning
    strategy for the system player, the sequence of configurations
    above satisfy the parity condition of the single-sided VASS game,
    so $\symbval_{l+1} \symbval_{l+2} \cdots$ symbolically satisfies
    $\phi$. From Lemma~\ref{lem:symbolicToConcreteSat} (symbolic
    vs.~concrete models), we conclude that $\sigma$ satisfies
    $\phi$.

\subsection{Proof details of Theorem~\ref{thm:ssVASSGamesToGRV}}
Given a single-sided VASS game, we
will make the following assumptions about it without loss of
generality.
\begin{itemize}
    \item The initial state belongs to the environment player (if it
        doesn't, we can add an extra state and a transition to achieve
        this).
    \item The environment and system players strictly alternate (if
        there are transitions between states belonging to the same
        player, we can add a dummy state belonging to the other player
        in between).
    \item The initial counter values are zero (if they aren't, we can
        add extra transitions before the initial state and force the
        system player to get the counter values from zero to the
        required values).
\end{itemize}

The formula giving the winning condition of the single-sided \pmainlogic[$\top$,
$\oblieqlocal$, $\leftarrow$] game is made up of the following variables. Suppose $T^e$ and $T^s$
are the sets of environment and systems transitions respectively. For every
transition $t \in T^e$, there is an environment variable $p_t$. We
indicate that the environment player chooses a transition $t$ by
setting $p_t$ to true.
For every transition $t \in T^s$ of the single-sided VASS game, there
is a system variable $t$. There is a
system variable $\curtrs$ to indicate the moves made by the
system
player. We indicate that the system player chooses a
transition $t$ by mapping $t$ and $\curtrs$ to the same data value. For every counter $x$ of the single-sided VASS game, there are
system variables $x$ and $\overline{x}$.

The formula $\phi_{e}$ indicates that the environment player makes
some wrong move and it is the disjunction of the following formulas.
\begin{itemize}
    \item The environment does not choose any transition in some
        round.
        \begin{align*}
            F(~ \bigwedge_{t \in T^{e}} \lnot p_t~)
        \end{align*}
    \item The environment chooses more than one transition in some
        round.
        \begin{align*}
            F (~ \bigvee_{t\ne t' \in T^{e}} ( p_t 
            \land p_{t'}) ~)
        \end{align*}
    \item The environment does not start with a transition originating
        from the designated initial state.
        \begin{align*}
            \bigvee_{t \in T^{e}, \text{ origin of } t \text{ is not
            the initial state}} p_t
        \end{align*}
    \item The environment takes some transition that cannot be
        taken after the previous transition by the system player.
        \begin{align*}
            \bigvee_{t \in T^{s}} F(~ t \oblieqlocal \curtrs ~ \land
            \bigwedge_{t' \in T_{s}\setminus \set{t}} \lnot (t'
            \oblieqlocal \curtrs) ~ \land \\ ~ \bigvee_{t' \in
                T^{e},~ t' \text{ can not come after } t}
                \mynext( p_{t'}) ~)
        \end{align*}
\end{itemize}

For simulating a counter $x$, we use two variables $x$ and
    $\overline{x}$. The data
    values assigned to these variables from positions $1$ to
    $i$ in a concrete model $\sigma$ will represent the counter value
that is
    equal to the cardinality of the set $\set{d \in \Domain \mid \exists j
    \in \set{1, \ldots, i}, \sigma(j)(x)=d, \forall j' \in \set{1, \ldots, i},
    \sigma(j')(\overline{x}) \ne d}$.  We will use special formulas for
    incrementing, decrementing and retaining previous values of
    counters.
\begin{itemize}
        \item To increment a counter represented by $x, \overline{x}$,
            we force the next data values of $x$ and $\overline{x}$ to
            be new ones that have never appeared before in $x$ or
            $\overline{x}$.
            \begin{align*}
                \phi_{\inc}(x, \overline{x}) = \mynext \lnot
(&~(\toblieqp{x}{x}) ~ \lor~
                (\toblieqp{x}{\overline{x}})~\lor ~
(\toblieqp{\overline{x}}{x})
                ~ \lor~\\ & ~
                (\toblieqp{\overline{x}}{\overline{x}}) ~ \lor ~ (x
\oblieqlocal
                \overline{x})~)
            \end{align*}
        \item To decrement a counter represented by $x,
            \overline{x}$, we force the next position to have a data
            value for $x$ and $\overline{x}$ such that it has appeared
            in the past for $x$ but not for $\overline{x}$.
            \begin{align*}
                \phi_{\dec}(x, \overline{x}) =& \mynext (~ x
\oblieqlocal
                \overline{x} ~ \land~ \toblieqp{x}{x} ~\land ~ \lnot
                (\toblieqp{x}{\overline{x}}) ~)
            \end{align*}
        \item To ensure that a counter represented by $x,
            \overline{x}$ is not changed, we force the next position
            to have a data value for $x$ that has already appeared in
            the past for $x$ and we force the next position to have a
            data value for $\overline{x}$ that has never appeared in
            the past for $x$ or $\overline{x}$.
            \begin{align*}
                \phi_{\nci}(x, \overline{x}) = \mynext(~
                \toblieqp{x}{x} ~ \land ~
                \lnot(\toblieqp{\overline{x}}{x}) ~ \land ~
                \lnot(\toblieqp{\overline{x}}{\overline{x}}) ~)
            \end{align*}
\end{itemize}

The formula $\phi_{s}$ indicates that the system player makes all the
right moves and it is the conjunction of the following formulas.
\begin{itemize}
    \item The system player always chooses at least one move.
        \begin{align*}
            G(~ \bigvee_{t \in T^{s}} t \oblieqlocal \curtrs ~)
        \end{align*}
    \item The system player always chooses at most one move.
        \begin{align*}
            G(~ \bigwedge_{t\ne t' \in T^{s}} \lnot(t \oblieqlocal
            \curtrs \land t' \oblieqlocal \curtrs) ~)
        \end{align*}
    \item The system player always chooses a transition that can come
        after the previous transition chosen by the environment.
        \begin{align*}
            \bigwedge_{t \in T^{e}}G(~ p_t ~
            \Rightarrow ~ \bigvee_{t'\in T_{s},~t' \text{ can come
            after } t}t' \oblieqlocal \curtrs  ~)
        \end{align*}
    \item The system player sets the initial counter values to zero.
        \begin{align*}
            \bigwedge_{x \text{ is a counter}}x \oblieqlocal
            \overline{x}
        \end{align*}
    \item The system player updates the counters properly.
        \begin{align*}
            G(~ & \bigwedge_{(q, x++,q')=t \in T^{s}} (~ t
\oblieqlocal
            \curtrs ~\Rightarrow ~ \phi_{\inc}(x, \overline{x})~ \land
            \bigwedge_{x' \ne x} \phi_{\nci}(x',\overline{x'}))\\
            &\bigwedge_{(q,\nop,q')=t\in T^{s}} (~ t\oblieqlocal
            \curtrs ~ \Rightarrow ~ \bigwedge_{x \text{ is a counter}}
            \phi_{\nci}(x,\overline{x}) ~)\\
            & \bigwedge_{(q, x--,q')=t \in T^{s}} (~ t \oblieqlocal
            \curtrs ~\Rightarrow ~ \phi_{\dec}(x, \overline{x})~ \land
            \bigwedge_{x' \ne x} \phi_{\nci}(x',\overline{x'}))~)
        \end{align*}
    \item The maximum colour occurring infinitely often is even.
        \begin{align*}
            \bigvee_{j \text{ is an even colour}} GF(\bigvee_{t\in T^e,
            \text{origin of } t \text{ has colour } j}(p_t) \\ \lor  \bigvee_{t\in T^s,
            \text{origin of } t \text{ has colour } j}(t
\oblieqlocal \curtrs))~ \land\\
             FG(\bigwedge_{t \in T, \text{ origin of } t \text{ has
colour greater than }
        j}\lnot( p_t \lor t \oblieqlocal \curtrs))
        \end{align*}
\end{itemize}

The system player wins if the environment player makes any mistake or
the system player makes all the moves correctly and satisfies the
parity condition. We set the winning condition for the system player
in the single-sided \pmainlogic[$\top$, $\oblieqlocal$, $\leftarrow$] game to be $\phi_{e} \lor
\phi_{s}$. If the system player has a winning strategy in the
single-sided VASS game, the system player simply makes choices in the
single-sided \pmainlogic[$\top$, $\oblieqlocal$, $\leftarrow$] game to
imitate the moves in the single-sided VASS game. Since the resulting
concrete model satisfies $\phi_{e} \lor \phi_{s}$, the system player
wins. Conversely, suppose the system player has a winning strategy in
the single-sided \pmainlogic[$\top$, $\oblieqlocal$, $\leftarrow$] game. In
the case where the environment does not make any mistake, the system
player has to choose data values such that the simulated sequence of
states of the VASS satisfy the parity condition.  Hence, the system
player in the single-sided VASS game can follow the strategy of the
system player in the single-sided \pmainlogic[$\top$, $\oblieqlocal$,
$\leftarrow$] game and irrespective of how the environment player plays, the
system player wins.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> app-undec-plrvgame.tex <==


\subsection{Proof details of Lemma~\ref{lem:undec-plrvgame-withbool}}
To simulate
counters $\countx$ and $\county$, we use the environment variable $x$
and system variable $y$. Suppose $\sigma$ is
the concrete model built during a game. The value of counter $\countx$
(resp.~$\county$) before the $i$\textsuperscript{th} transition is the
cardinality of the set $\set{d \in \Domain \mid \exists j \in \set{1,
\ldots, i}: \sigma(j)(x)=d, \forall j' \in \set{1, \ldots, i}:
\sigma(j')(y) \ne d}$ (resp.~$\set{d \in \Domain \mid \exists j \in
\set{1, \ldots, i}, \sigma(j)(y)=d, \forall j' \in \set{1, \ldots,
i}, \sigma(j')(x) \ne d}$). Intuitively, the value of counter
$\countx$ is the number of data values that have appeared under
variable $x$ but not under $y$. To increment $\countx$, a fresh new
data value is assigned to $x$ and the data value assigned to
$y$ should be one that has already appeared before under $x$ and
$y$. To decrement $\countx$, the same data value should be assigned to
$x$ and $y$ and it should have appeared before under $x$ but not under
$y$. In order to test that $\countx$ has the value zero, the same data
value should be assigned to $x$ and $y$. In addition, every increment
for $\countx$ should have been matched by a subsequent decrement for
$\countx$. The operations for $\county$ should follow similar rules,
with $x$ and $y$ interchanged.

For
every transition $t$ of the 2-counter machine, there is a Boolean
variable $p_t$ owned by \env. The $i$\textsuperscript{th} transition
chosen by \env is in the $(i+1)$\textsuperscript{st} valuation. The
set $\Phi^e$ consists of the following formulas, each of which denotes
a mistake made by \env.
\begin{itemize}
\item \env chooses some transition in the first position.
\begin{align*}
\bigvee_{t \text{ is any transition}} p_t
\end{align*}
\item The first transition is not an initial transition.
\begin{align*}
\mynext (\bigvee_{t \text{ is not an initial transition}} p_t)
\end{align*}
\item \env chooses more or less than one transition.
\begin{align*}
  \mynext F( \bigvee_{t \ne t'} (p_t \land p_{t'}) \lor \bigwedge_{t\text{ is any
transition}}(\lnot p_t))
\end{align*}
\item Consecutive transitions are not compatible.
\begin{align*}
\mynext F( \bigvee_{t' \text{ cannot come after } t} (p_t \land \mynext
p_{t'}))
\end{align*}
\item A transition increments $x$ but the data value for $x$ is old.
\begin{align*}
\mynext F (\bigvee_{t \text{ increments } x} p_t \land (\toblieqp{x}{x}
\lor \toblieqp{x}{y}))
\end{align*}
\item A transition decrements $x$ but the data value for $x$ has not
appeared under $x$ or it has appeared under $y$.
\begin{align*}
\mynext F (\bigvee_{t \text{ decrements } x} p_t \land (\lnot
\toblieqp{x}{x} \lor \toblieqp{x}{y}) )
\end{align*}
\item A transition increments $c_y$ but the data value for $x$ is
new.
\begin{align*}
\mynext F (\bigvee_{t \text{ increments } y} p_t \land 
(\lnot \toblieqp{x}{x} \lor \lnot \toblieqp{x}{y}))
\end{align*}
\item A transition decrements $c_y$ but the data value for $x$ has not
    appeared before in $y$ or it has appeared before in $x$.
\begin{align*}
\mynext F (\bigwedge_{t \text{ decrements } y} p_t \land (\lnot
(\toblieqp{x}{y}) \lor \toblieqp{x}{x}))
\end{align*}
\item A transition tests that the value in the counter $c_x$ is zero,
but there is a data value that has appeared under $x$ but not under
$y$. In such a case, \sys can map that value to $y$, make the
following formula true and win immediately.
\begin{align*}
\mynext F ( \bigvee_{t \text{ tests } c_x \text{ for } 0} p_t \land
\toblieqp{y}{x} \land \lnot \toblieqp{y}{y})
\end{align*}
\item A transition tests that the value in the counter $c_y$ is zero,
but there is a data value that has appeared under $y$ but not under
$x$. In such a case, \sys can map that value to $y$, make the
following formula true and win immediately.
\begin{align*}
\mynext F ( \bigvee_{t \text{ tests } c_y \text{ for } 0} p_t \land
\toblieqp{y}{y} \land \lnot \toblieqp{y}{x})
\end{align*}
\end{itemize}

The set $\Phi^s$ consists of the following formulas, each of which
denotes constraints that \sys has to satisfy after \env makes a move.
\begin{itemize}
\item If a transition increments $c_x$, then the data value of $y$ must
already have appeared in the past.
\begin{align*}
\mynext G ( \bigwedge_{t \text{ increments } c_x} ( p_t \Rightarrow (
\toblieqp{y}{x} \land \toblieqp{y}{y})))
\end{align*}
\item If a transition increments $c_y$, then the data value of $y$ must
be a fresh one.
\begin{align*}
\mynext G( \bigwedge_{t \text { increments } c_y} p_t \Rightarrow \lnot
(y \oblieqlocal x) \land \lnot (\toblieqp{y}{x}) \land \lnot
(\toblieqp{y}{y}))
\end{align*}
\item If a transition decrements $c_x$ or $c_y$ or tests one of them
    for zero, then the data value of $y$ must
be equal to that of $x$.
\begin{align*}
\mynext G( \bigwedge_{t \text { decrements/zero tests some counter}} p_t \Rightarrow y
\oblieqlocal x)
\end{align*}
\item The halting state is reached.
    \begin{align*}
        \mynext F \bigvee_{t \text{ is a transition whose target state
        is halting}} p_t
    \end{align*}
\end{itemize}
The winning condition of the \pmainlogic[$\top$, $\oblieqlocal$,
$\leftarrow$] game is given by the formula $\bigvee \Phi^{e} \lor
\bigwedge \phi^{s}$. For \sys to win, one of the formulas in
$\Phi^e$ must be true or all the formulas in $\Phi^s$ must be true.
Hence, for \sys to win, \env should make a mistake during simulation
or no one makes any mistake and the halting state is reached. Hence,
\sys has a winning strategy iff the 2-counter machine reaches the
halting state.
%\paragraph{Correctness.}
%Remember that for simplicity we assume that the $2$-counter machines has a final state $q_f$ and contains a transition $\hat t = (q_f, \countx++,q_f)$, it is easy to see that this preserves the undecidability of the model. Suppose first that the $2$-counter machine has an accepting run $(q_0, I_1,q_1) \dotsb (q_{n-1},I_n,q_n)$ with $q_n=q_f$. \Sys{}'s strategy is then to play (the encoding of) the labels 
%\[\textit{begin} \, (q_0, I_1,q_1) \dotsb (q_{n-1},I_n,q_n) \, \hat t^\omega.\]
%In this way, formulas $\phi_1$ and $\phi_2$ will be true.
%With respect to the data values on $x$, \sys will consistently play any data value at the first round, and at the $i+1$ round a fresh data value if $I_i = \countx++$, a data value that has appeared under $x$ but not under $y$ if $I_i = \countx--$, and a data value that has appeared under $x$ otherwise. This playing strategy makes all the formulas $\phi_3, \dotsc, \phi_7$ true.
%
%\Env is, on the other hand, constrained to play a fresh data value for $I_i = \county++$ an old $y$-value if $I_i = \county--$ and to play the same data value as \sys if $I_i = (\countx =0?)$ or $I_i = (\county=0?)$. If \env does not do so, then $\phi_A \land \dotsb \land \phi_E$ would be false, and the property would hold true, allowing \sys to win the play.
%
%Finally, the fact that the labels come from correct run of the 2-counter machine ensures that there are no tests for zero for a non-zero-valued counter, and thus any data value  \env plays at a test for zero label will either be an old $y$-value making false $\phi_I$
%
%neither $\phi_{I}$ nor $\phi_{II}$ can ever hold true, irrespective of what \env plays.
%
%\smallskip
%
%On the other hand, if the $2$-counter machine cannot reach the target state $q_f$, then, assuming that \env plays as described before, and \sys finds a way to verify $\phi_1 \land \dotsc, \phi_7$, then necessarily there will be either: a decrement of a zero-valued counter, in which case $\phi_1$ is true; or a test for zero of a non-null counter, in which case $\phi_2$ is true. Thus, there cannot be a strategy for \sys that makes the property hold true.

\subsection{Proof details of Lemma~\ref{lem:undec-plrvgame-nobool}}

Indeed, note that assuming this encoding, we can make sure that we are standing at the left boundary of a block using the \pmainlogic{} formula
\[\phi_{\textit{block}(0)} = (x \oblieqlocal \mynext^{m+3}x) \land x \oblieqlocal \mynext x;
\]
and we can then test that we are in position $i\in \set{1, \dotsc, m+2}$ of a block through the formula
\[
\phi_{\textit{block}(i)}=\mynext^{-i} \phi_{\textit{block}(0)}.
\]

For any fixed linear order on the set of labels $\lambda_1 < \dotsb < \lambda_{m-1}$, we will encode that the current block has the $i$-th label $\lambda_i$ as
\[
\phi_{\lambda_i} = \phi_{\textit{block}(0)} \land \mynext^2(x \oblieqlocal \mynext^i x).
\]
Notice that in this coding of labels, a block could have several labels, but of course this is not a problem, if need be one can ensure that exactly one label holds at each block.
\[
\phi_{\textit{1-label}} = \bigvee_i \phi_{\lambda_i} \land \lnot \bigwedge_{i \neq j} \phi_{\lambda_i} \land \phi_{\lambda_j}
\] 
Also, observe that through a binary encoding one could encode the labels in blocks of logarithmic length.

Now the question is: How do we enforce this shape of data words?

Firstly, the structure of a block on variable $x$ can be enforced through the following formula
\begin{align*}
\phi_{\textit{block-str}} =~ &\mynext^2(\lnot (\toblieqp{x}{x})) ~\land\\
&\bigwedge_{1< i \leq m+1} \mynext^i ( (x \oblieqlocal \mynext^{1-i}x) \lor \lnot (\toblieqp{x}{x}))  ~\land\\
& \phi_{\textit{1-label}} \land  \mynext^{m+1}( x \oblieqlocal \mynext x).
\end{align*}
The first two lines ensure that the data values of each $w_i$ are `fresh' (\ie, they have not appeared before the current block); while the last line ensures that the two last positions repeat the data value and that each blocks encodes exactly one label.
Further, a formula can inductively enforce that this structure is repeated on variable $x$:
\begin{enumerate}
\item[8)] The first position verifies $\phi_{\textit{block}(0)}$; and for every position we have $\phi_{\textit{block}(0)} \Rightarrow \phi_{\textit{block-str}} \land \mynext^{m+2}\phi_{\textit{block}(0)}$ 
\end{enumerate}

And secondly, we can make sure that the $y$ variable must have the same data value as the $x$ variable in all positions ---except, of course, the $(m+3)$-rd positions of blocks. This can be enforced by making false the formula as soon as the following property holds.
\begin{enumerate}
\item[F)] There is some $i \in \set{0,\dotsc, m+1}$ and some position verifying
  \[
    \phi_{\textit{block}(i)} \land \lnot (x \oblieqlocal y).
  \]
\end{enumerate}

In each of the formulas $\phi$ described in the previous section, consider now guarding all positions with $\phi_{\textit{block}(m+2)}$\footnote{That is, where it said ``there exists a position where $\psi$ holds'', now it should say ``there exists a position where $\phi_{\textit{block}(m+2)}\land \psi$ holds'', where it said ``for every position $\psi$ holds'' it should now say ``for every position $\phi_{\textit{block}(m+2)} \Rightarrow \psi$ holds''.}; replacing  each test for a label $\lambda_i$ with $\mynext^{-(m+2)}\phi_{\lambda_i}$; and replacing each $\mynext^i$ with $\mynext^{(m+3)i}$, obtaining a new formula $\hat\phi$ that works over the block structure encoding we have just described.

Then, for the resulting formula $\bigvee \hat\Phi^{e} ~ \lor ~
\bigwedge \hat\Phi^{s}$
%\[
%\phi' = \lnot\hat \phi_A \land \dotsb \land \lnot \hat \phi_E \land \lnot \phi_F \Rightarrow  
%\hat \phi_1 \land \dotsb \land \hat \phi_7 \land \phi_8 \land \lnot \hat \phi_{\text{I}} \land \lnot \hat \phi_{\text{II}} 
%\]
there is a winning strategy for \sys if, and only if, there is an accepting run of the 2-counter machine.


\subsection{Proof details of Lemma~\ref{lem:undec-plrvgame-nolocal}}
In the reduction from Lemma~\ref{lem:undec-plrvgame-nobool}, one can use the following encoding to replace testing whether two  positions at distance $n$ have the same data value with a chained series of tests.
Each block of the form 
\[
  \begin{array}{rlllllllllll}
    x:&d&d&d_1&d_2&d_3&d_4& \dotsb &d_m&x_i&d&d\\
    y:&d&d&d_1&d_2&d_3&d_4& \dotsb &d_m&y_i&d&d
  \end{array}
\]
will now look like:
\[\arraycolsep=2.87pt\def\arraystretch{1}
  \begin{array}{rlllllllllllllllll}
    x:&d&d&d_1&d_2&d&d_1&d_3&d&d_1&d_4& \dotsb &d&d_1&d_m&x_i&d&d\\
    y:&d&d&d_1&d_2&d&d_1&d_3&d&d_1&d_4& \dotsb &d&d_1&d_m&y_i&d&d
  \end{array}
\]
Note that $d,d_1$ repeats along the whole block in such a way that testing if $d_i = d_1$ and ensuring that the first two data values are equal to the last two data values can be done using data tests of bounded $\mynext$-distance. Therefore, determining the winner of a \pmainlogic{} game is still undecidable if both the variables and the $\mynext$-distance is bounded.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> app-undec-singlesided-plrvgame.tex <==

We briefly discuss why the properties $\phi_{\textit{lab}}$, $\phi_{x,y}$, $\psi_1$ and $\psi_2$ can be described in \pmainlogic$[\top, \oblieqlocal, \leftarrow]$. 

Encoding $\phi_{\textit{lab}}$ using some Boolean variables belonging to \sys is easy since it does not involve the use of data values. 

The formula $\phi_{x,y}$ can be encoded as $\always(\bigwedge_{a \in A} \tau_{a} \Rightarrow \zeta_{a})$ for $A = \set{\countx++, \countx--, \countx = 0?, \county++, \county--, \county = 0?}$ and 
\[\tau_a = \bigvee_{q,q' \in Q, (q,a,q') \in \delta} \lambda_{(q,a,q')},\] where $\lambda_{(q,a,q')}$ tests that we are standing on a position labelled with transition $(q,a,q')$ (in particular not a \emph{bis} position). Finally, $\zeta_a$ encodes the rules as already described. That is, 
\begin{align*}
  \zeta_{\countx++} = {}&x \oblieqlocal y \land x \oblieqlocal \mynext x \land y
  \oblieqlocal \mynext y \land \lnot \mynext(\toblieq{x}{y} ),\\
  \zeta_{\countx--} = {}&\lnot x \oblieqlocal y \land \lnot \toblieq{x}{x} \land \lnot \toblieq{x}{y} \land {} \\
& y \oblieqlocal \mynext y \land y \oblieqlocal \mynext x,\\
  \zeta_{\countx=0?} = {}&x \oblieqlocal y \land x \oblieqlocal \mynext x \land y \oblieqlocal \mynext y,
\end{align*}
and similarly for the rules on $\county$.

The formula $\psi_1 = \mu \land ( (\pi_1 \land \lnot \pi'_1) \Rightarrow (\phi_1 \land \lnot \phi'_1))$ is actually composed of two conjunctions $\psi_1 = \psi_1^x \land \psi_1^y$, one for $k=x$ and another for $k=y$, let us first suppose that $k=x$. Then,
\begin{itemize}
\item $\pi_1$, which checks Property 1, which is simply 
\[
\pi_1 = b \until (\lnot b \land \tau_{\countx = 0?} \land \mynext(\lnot b \until \tau_{\countx--}))
\]
%
\item $\pi'_1$, expresses that there exists a $\countx ++$ with $\lnot b$ with value matching that of a future $z$-value:
\[
\pi'_1 = \future(\tau_{\countx++} \land \lnot b \land \toblieq{x}{z})
\]
%
\item $\phi_1$, on the other hand, checks that $z$ carries always the same data value, disjoint from the values of all other variables, but  as soon as the last $\bot$ value is played the value of $z$ in the next position changes and holds now the $x$ value of that position, and it continues to hold it forever:
  \begin{align*}
\phi_1 = {} &\lnot (\toblieq{z}{x} \lor \toblieq{z}{y}) \land {}\\
&(z \oblieqlocal \mynext z )\until \big(\lnot(z \oblieqlocal \mynext z) \land\lnot b \land \mynext b  \land  x \oblieqlocal \mynext z \land \mynext\always(z \oblieqlocal \mynext z)\big)
  \end{align*}
%
\item finally, $\phi'_1$  tests there exists a $\countx ++$ transition whose principal value corresponds to the $z$-value of some future position:
  \begin{align*}
    \phi'_1 &= \future (\tau_{\countx++} \land \toblieq{x}{z}).
  \end{align*}
\end{itemize}






The formula $\psi_2 = \pi_2 \Rightarrow \phi_2 \land \phi'_2$ is also composed of two conjuncts, one for $k=x$ and one for $k=y$, let us only show the case $k=x$. Then,
\begin{itemize}
\item $\pi_2$ checks Property 2:
\[
\pi_2 = b \until (\lnot b \land \tau_{\countx--} \land \mynext(\always b))
\]
%
\item $\phi_2$ checks  that as soon as $b$ turns to $\bot$ then $z$ at the next position takes the value as current variable $x$, and maintains that value:
  \begin{align*}
\phi_2 = {} &\lnot (\toblieq{z}{x} \lor \toblieq{z}{y}) \land {}\\
&(z \oblieqlocal \mynext z )\until \big(\lnot(z \oblieqlocal \mynext z) \land \lnot b  \land  x \oblieqlocal \mynext z \land \mynext\always(z \oblieqlocal \mynext z)\big)
  \end{align*}
%
\item finally, $\phi'_2$  tests that in this situation there must be some $\countx++$ position with a data value equal to variable $z$ of a future position:
  \begin{align*}
    \phi'_2 &= \future (\tau_{\countx++} \land \toblieq{x}{z}).
  \end{align*}
\end{itemize}


\paragraph{Correctness.} 
Suppose first that the $2$-counter machine has an accepting run $(q_0, I_1,q_1) \dotsb (q_{n-1},I_n,q_n)$ with $q_n=q_f$. \Sys{}'s strategy is then to play (the encoding of) the labels 
\[(q_0, I_1,q_1) \, \textit{bis}\, \dotsb (q_{n-1},I_n,q_n) \, \textit{bis}\, (\hat t \, \textit{bis})^\omega.\]
In this way, the formula $\phi_{\textit{lab}}$ holds.

With respect to the data values on $x,y$, \sys will respect the rules depicted in Section~\ref{undec-singlesided-plrvgame}, making $\phi_{x,y}$ true.

Finally, \sys will play a data value in $z$ that at the beginning will be some data value which is not used on variables $x$ nor $y$. She will keep this data value all the time, but keeping an eye on the value of $b$ that is being played by \env. If \env plays a first $\bot$ on a $c_k--$ transition, \sys will then play on $z$, at the next round, the data value of variable $k$ at this round. If \env plays a first $\bot$ at a $c_k=0?$ transition and a last $\bot$ at a $c_k--$ transition, again \sys will change the value of $z$ to have the principal value of the $c_k--$ transition. In this way, \sys is sure to make true the formula $\phi_1 \land \lnot \phi_1'$ in one case, and formula $\phi_2 \land \phi'_2$ in the other case. All other cases for $b$ are going to be winning situations for \sys due to the preconditions $\pi_1 \land \lnot \pi'_1$ and $\pi_2$ in the formulas $\psi_1$ and $\psi_2$.

\smallskip

On the other hand, if there is no accepting run for the $2$-counter machine, then each play of \sys on variables $x,y$ and the variables verifying both $\phi_{\textit{lab}}$ and $\phi_{x,y}$ must have an illegal transition of type a) or b). At the first illegal transition \env will play $\bot$. If it is a $c_k--$ illegal transition, then \env will continue playing $\top$ in subsequent positions; if it is a $c_k=0?$ illegal transition, then \env will keep playing $\bot$ until the corresponding $c_k--$ matching to a witnessing $c_k++$ played before the $c_k=0?$ transition is reached. In either of these situations the antecedent of $\psi_1$ or $\psi_2$ will be true while the consequent will be false; and thus the final formula will not hold, making \sys incapable of finding a winning strategy.

\smallskip

Finally, let us explain further how this reduction can be turned into a reduction for the game in which \env plays first and \sys plays second at each round. For the final formula $\phi$ of the reduction, let $\phi'$ be the formula in which \env conditions are shifted one step to the right. This is simply done by replacing every sub-expression of the form $\mynext^i b$ with $\mynext^{i+1}b$. It follows that if \env starts playing $\top$ and then continues the play reacting to \sys strategy in the same way as before, \sys will have no winning strategy if, and only if, \sys had no winning strategy in the game where the turns are inverted.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

